IMRank: Influence Maximization via Finding Self-Consistent Ranking

Influence maximization, fundamental for word-of-mouth marketing and viral marketing, aims to find a set of seed nodes maximizing influence spread on social network. Early methods mainly fall into two paradigms with certain benefits and drawbacks: (1)Greedy algorithms, selecting seed nodes one by one, give a guaranteed accuracy relying on the accurate approximation of influence spread with high computational cost; (2)Heuristic algorithms, estimating influence spread using efficient heuristics, have low computational cost but unstable accuracy. We first point out that greedy algorithms are essentially finding a self-consistent ranking, where nodes' ranks are consistent with their ranking-based marginal influence spread. This insight motivates us to develop an iterative ranking framework, i.e., IMRank, to efficiently solve influence maximization problem under independent cascade model. Starting from an initial ranking, e.g., one obtained from efficient heuristic algorithm, IMRank finds a self-consistent ranking by reordering nodes iteratively in terms of their ranking-based marginal influence spread computed according to current ranking. We also prove that IMRank definitely converges to a self-consistent ranking starting from any initial ranking. Furthermore, within this framework, a last-to-first allocating strategy and a generalization of this strategy are proposed to improve the efficiency of estimating ranking-based marginal influence spread for a given ranking. In this way, IMRank achieves both remarkable efficiency and high accuracy by leveraging simultaneously the benefits of greedy algorithms and heuristic algorithms. As demonstrated by extensive experiments on large scale real-world social networks, IMRank always achieves high accuracy comparable to greedy algorithms, with computational cost reduced dramatically, even about $10-100$ times faster than other scalable heuristics.

==> imrank_section.implements.tex <==
\section{Implementation of IMRank}\label{section:implement}

In the implementation of IMRank, there are two aspects need to be more concrete: one is the influence propagation network construction method; another is the initial ranking strategy, or initial sort.

\subsection{Influence propagation network}

In this section, we focus on the construction of rank-based influence propagation network from the original influence network. As we discussed in the above section, the influence propagation network is consisted of different influence propagation paths. With respect to calculate rank-based influence, the influence can not be propagated from a node to other nodes ranked higher than itself. Hence, for a directed edge $\langle u,v\rangle$ exists in the original influence network, if $v$ is ranked higher than $u$, then this edge should be \emph{blocked} from the rank-based influence propagation network. After removing such edges, the obtained influence network will become a tree structure and is always much sparser than the original influence network.

However, even after blocking all those edges out from a node with low rank to a node with high rank, the computational complexity for considering all the remained paths is still expensive. Actually, most of these paths are with low propagation probabilities and unimportant. Hence, we use local influence to estimate the global rank-based influence.

For a path $P(u,v)=\langle u=w1,w2,\ldots,w_m=v\rangle$, we denote the distance of this path as $d(P)$, and the propagation probability of the path as $pp(P)$, then there are $d(P)=m-1$ and $pp(P)=\prod_{i=1}^{m-1}p(w_i,w_{i+1})$. Based on the two concepts, we suggest two ways to obtain a local influence propagation network for each node as follows:
%with propagation probability on each edge$\langle w_i,w_{i+1}\rangle$ is $p(w_i,w_{i+1})$

\begin{itemize}
  \item \textbf{Distance-based construction}: for each node $u$, we only consider its influence to the nodes with distance no more than an integer $l(l\geq1)$ from it, i.e., only consider every influence propagation path starting from it to a node $v$ with $d(P(u,v))\leq l$. When $l=1$, it means that, only the direct influence of a node is considered. When $l>1$, indirect influence of a node will be considered. For the influence score allocation process, it is the exact opposite of influence propagation process. Hence, $u$ needs to allocate its influence score through every path with $d(P(w,u))\leq l$ to $w$. %In this case, a node only need to allocate its influence score to its directed parent node with rank higher than itself.  %a node can only influence its direct child nodes
  \item \textbf{Influence-based construction}: for each node $u$, we only consider its influence propagation paths with propagation probabilities larger than an influence threshold $\theta(0<\theta<1)$, i.e., $pp(P(u,v))>\theta$, and it needs to allocate its influence score through all the paths with $pp(P(w,u))>\theta$. This influence threshold $\theta$ is used to eliminate propagation paths that have too small propagation probabilities. A smaller $\theta$ always leads to more accurate influence network. %In this construction, a node need to allocate its influence score through all the influence propagation paths with propagation probability larger than $\theta$.
\end{itemize}

Besides, according to bottom-up strategy, there are lots of paths can be further safely neglected. Figure~\ref{negelectPath} gives an example for paths can be safely neglected. Supposing the current rank is $L=\{v_1,v_2,v_3, v_4,v_5,v_6,v_7\}$. With respect to $v_6$, when considering all the influence propagation paths with $d(P)\leq2$, the path $\langle v_1,v_4,v_6\rangle, \langle v_3,v_5,v_6\rangle$ can be neglected. $v_6$ only needs to consider the paths $\langle v_4,v_6\rangle$ and $\langle v_5,v_6\rangle$, and allocates influence score to node $v_4$ and $v_5$. That's because the edges forming those paths are all \emph{unblocked}, i.e., influence can propagate normally, and the influence score can be sent normally through the intermediate nodes. While for the path $\langle v_2,v_7,v_6\rangle$, since $v_7$ is ranked lower than $v_6$, the edge $\langle v_7, v_6\rangle$ is blocked, the influence score can not be sent through $v_7$ to $v_2$, hence $\langle v_2,v_7,v_6\rangle$ can not be neglected. From the above example, it is clearly that, if an influence path is consisted of unblocked edges, the node only needs to send influence score to its direct parent in this path. Hence, when a node collects the set of paths to allocate influence score through, when it reaches a node ranked higher than itself and satisfy the construction requirement, there is no need to continue search the parent nodes of this parent node.

\begin{figure}
\centering
\includegraphics[width=0.2\textwidth]{pics/neglectPaths.eps}
\caption{The influence paths will be considered in rank-based influence calculation. }
\label{negelectPath}
\end{figure}

%The complexity of our algorithm hasn't been analysis, for the ranking
%Obviously, the influence score allocated to a node more related to its present rank but not its score in the marginal influence calculation. This is just the reason why existing diversity algorithms can not be directly used for influence maximization, while our algorithm is designed specially for influence maximization.


\subsection{Initial rank}\label{section:initalRank}
With regard to IMRank, the initial rank intuitively has impacts on the final converged rank. It is due to that, rank-based influence has rank preference. A node can only receive influence score from the nodes ranked lower than itself. Hence, the rank-based influence calculation is strong negative to the nodes ranked low in the initial ranking. Those nodes are always difficult to make substantial changes to their initial ranks.

From the above analysis, it is easy to conclude that, a sort with the influence preference will be suitable as the initial sort for IMRank. There the influence preference means that, influential nodes are ranked high in this sort. Essentially, IMRank is to quickly optimize the initial sort to be a well sorted set for influence maximization, and aims to balance the influence and influence overlap of top ranked nodes. Hence, a suitable initial ranking strategy for IMRank should have certain influence preference. An initial ranking method with none such preference, such as a random generated sorted set, or with reverse influence preference will certainly limit the performance of IMRank.

Based on the above analysis, we suggest six simple initial ranking methods. All of those ranking methods obtain a sort with certain influence preference. They are:
\begin{itemize}
  \item \textbf{OutDegree}: to rank nodes simply by the out degree;
  \item \textbf{WeightedOutDegree}: to rank nodes by the weighted out degree, which is the sum of the propagation probability on all the out edges of a node;
  \item \textbf{PageRank}: the classical rank used for ranking webpages~\cite{Brin1998}. We set the parameter damping factor $\alpha$ of this ranking method to 0.15, and the stopping criteria is when the average differ of the scores of each node in two consecutive iterations is at most $10^{-1}$.
  \item \textbf{IR}: to rank nodes by the score calculated by heuristic iteratively ranking strategy proposed in ~\cite{Jung2012}. We set the parameters $\alpha$ and $\theta$ as 0.7 and $1/320$, and set the maximum times of iterations to 20;
  \item \textbf{SameLocalRank}: to rank nodes by the score received by each node in the case that every node sends influence score to their direct parent nodes equally as those parent nodes have the same rank;
  \item \textbf{RandomLocalRank}: to rank nodes by the score received by each node in the case that each node sends influence score to its direct parent nodes according to a randomly generated rank by itself;
\end{itemize}

Actually, IMRank is indeed relative insensitive to different initial ranking methods. We will show that experimentally in Section~\ref{section:experiment}. Simple ranking methods, such as Degree, PageRank, can meet the requirement of influence preference. Combined with all those initial ranks, IMRank can always achieve a solution with high influence spread very close to Kempe's greedy algorithm and other heuristics.

